An Empirical Study on Capability of Large Language Models in Understanding Code Semantics

Large Language Models for Code (code LLMs) have demonstrated remarkable performance across various software engineering (SE) tasks, increasing the application of code LLMs in software development. Despite the success of code LLMs, there remain significant concerns about the actual capabilities and reliability of these models, "whether these models really learn the semantics of code from the training data and leverage the learned knowledge to perform the SE tasks". In this paper, we introduce EMPICA, a comprehensive framework designed to systematically and empirically evaluate the capabilities of code LLMs in understanding code semantics. Specifically, EMPICA systematically introduces controlled modifications/transformations into the input code and examines the models' responses. Generally, code LLMs must be robust to semantically equivalent code inputs and be sensitive to non-equivalent ones for all SE tasks. Specifically, for every SE task, given an input code snippet c and its semantic equivalent variants, code LLMs must robustly produce consistent/equivalent outputs while they are expected to generate different outputs for c and its semantic non-equivalent variants. Our experimental results on three representative code understanding tasks, including code summarization, method name prediction, and output prediction, reveal that the robustness and sensitivity of the state-of-the-art code LLMs to code transformations vary significantly across tasks and transformation operators. In addition, the code LLMs exhibit better robustness to the semantic preserving transformations than their sensitivity to the semantic non-preserving transformations. These results highlight a need to enhance the model's capabilities of understanding code semantics, especially the sensitivity property.

==> 5.results/tables-backup/rq2_methodname_em.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{RQ2. The exactly match of the method names generated by LLMs for the original program and the transformed program}
\label{tab:dependence_concepts}
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{l|l|l|rrr|rrr}
\toprule
                                                                                                                           & \multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{3}{c|}{\textbf{Java}}                                                                                                      & \multicolumn{3}{c}{\textbf{Python}}                                                                                                    \\ \cmidrule{4-9} 
\multirow{-2}{*}{}                                                                                                         & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Dependence}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Transformation \\ operator\end{tabular}}}} & \multicolumn{1}{c|}{DeepSeek}                     & \multicolumn{1}{c|}{Codellama}                    & \multicolumn{1}{c|}{MagicCoder} & \multicolumn{1}{c|}{DeepSeek}                     & \multicolumn{1}{c|}{Codellama}                    & \multicolumn{1}{c}{MagicCoder} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Convert \\ For/While\end{tabular}                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.72} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.81} & 0.85                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.60}     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.42}     &    0.53                             \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Control}          & \begin{tabular}[c]{@{}l@{}}Flip\\ IfElse\end{tabular}                                                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.80} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.59} & 0.83                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.53} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.47} & 0.67                            \\ \cmidrule{2-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Rename \\ variable\end{tabular}                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.34} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.40} & 0.52                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.32} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.32} & 0.36                            \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Semantic \\ Preserving \\ Transformation\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Data}             & \begin{tabular}[c]{@{}l@{}}Reorder \\ parameters\end{tabular}                                                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.72} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.56} & 0.63                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.66} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.53} & 0.66                            \\ \midrule
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ relational \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.45}                         & \multicolumn{1}{r|}{0.53}                         & 0.59                            & \multicolumn{1}{r|}{0.38}                         & \multicolumn{1}{r|}{0.46}                         & 0.50                            \\ \cline{3-9} 
                                                                                                                           & \multirow{-2}{*}{Control}                                  & \begin{tabular}[c]{@{}l@{}}Remove \\ conditional \\ statement\end{tabular}                                         & \multicolumn{1}{r|}{0.39}                         & \multicolumn{1}{r|}{0.35}                         & 0.38                            & \multicolumn{1}{r|}{0.28}                         & \multicolumn{1}{r|}{0.30}                         & 0.33                            \\ \cmidrule{2-9} 
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ arithmetic \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.49}                         & \multicolumn{1}{r|}{0.43}                         & 0.44                            & \multicolumn{1}{r|}{0.35}                         & \multicolumn{1}{r|}{0.30}                         & 0.37                            \\ \cmidrule{3-9} 
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}Semantic\\ Non-Preserving \\ Transformation\end{tabular}}                      & \multirow{-2}{*}{Data}                                     & \begin{tabular}[c]{@{}l@{}}Remove \\ def \\ statement\end{tabular}                                                 & \multicolumn{1}{r|}{0.51}                         & \multicolumn{1}{r|}{0.68}                         & 0.53                            & \multicolumn{1}{r|}{0.39}                         & \multicolumn{1}{r|}{0.62}                         & 0.55                            \\ \bottomrule
\end{tabular}
}
\end{table}

==> 5.results/tables-backup/rq2_methodname_f1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{RQ2. The similarity in terms of F1-score of the method names generated by LLMs for the original program and the transformed program}
\label{tab:dependence_concepts}
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{l|l|l|rrr|rrr}
\toprule
                                                                                                                           & \multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{3}{c|}{\textbf{Java}}                                                                                                      & \multicolumn{3}{c}{\textbf{Python}}                                                                                                    \\ \cmidrule{4-9} 
\multirow{-2}{*}{}                                                                                                         & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Dependence}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Transformation \\ operator\end{tabular}}}} & \multicolumn{1}{c|}{DeepSeek}                     & \multicolumn{1}{c|}{Codellama}                    & \multicolumn{1}{c|}{MagicCoder} & \multicolumn{1}{c|}{DeepSeek}                     & \multicolumn{1}{c|}{Codellama}                    & \multicolumn{1}{c}{MagicCoder} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Convert \\ For/While\end{tabular}                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.85} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.90}  & 0.93                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.82}     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.67}     &    0.77                             \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Control}          & \begin{tabular}[c]{@{}l@{}}Flip \\ IfElse\end{tabular}                                                             & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.91} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.78} & 0.94                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.8}  & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.7}  & 0.82                            \\ \cmidrule{2-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Rename \\ variable\end{tabular}                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.62} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.61} & 0.74                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.62} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.55} & 0.63                            \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Semantic \\ Preserving \\ Transformation\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Data}             & \begin{tabular}[c]{@{}l@{}}Reorder \\ parameters\end{tabular}                                                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.88} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.71} & 0.79                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.81} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.67} & 0.82                            \\ \midrule
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ relational \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.70}                          & \multicolumn{1}{r|}{0.75}                         & 0.8                             & \multicolumn{1}{r|}{0.69}                         & \multicolumn{1}{r|}{0.68}                         & 0.76                            \\ \cmidrule{3-9} 
                                                                                                                           & \multirow{-2}{*}{Control}                                  & \begin{tabular}[c]{@{}l@{}}Remove \\ conditional \\ statement\end{tabular}                                         & \multicolumn{1}{r|}{0.58}                         & \multicolumn{1}{r|}{0.59}                         & 0.56                            & \multicolumn{1}{r|}{0.56}                         & \multicolumn{1}{r|}{0.53}                         & 0.58                            \\ \cmidrule{2-9} 
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ arithmetic \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.66}                         & \multicolumn{1}{r|}{0.64}                         & 0.64                            & \multicolumn{1}{r|}{0.62}                         & \multicolumn{1}{r|}{0.5}                          & 0.63                            \\ \cmidrule{3-9} 
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}Semantic \\ Non-Preserving \\ Transformation\end{tabular}}                     & \multirow{-2}{*}{Data}                                     & \begin{tabular}[c]{@{}l@{}}Remove \\ def \\ statement\end{tabular}                                                 & \multicolumn{1}{r|}{0.75}                         & \multicolumn{1}{r|}{0.83}                         & 0.76                            & \multicolumn{1}{r|}{0.7}                          & \multicolumn{1}{r|}{0.75}                         & 0.75                            \\ \bottomrule
\end{tabular}
}
\end{table}

==> 5.results/tables-backup/rq2_output.tex <==



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{RQ2. The similarity of the outputs predicted by LLMs for the  original program and the transformed program}
\label{tab:dependence_concepts}
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{l|l|l|rrr|rrr}
\toprule
                                                                                                                           & \multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{3}{c|}{\textbf{Java}}                                                                                                      & \multicolumn{3}{c}{\textbf{Python}}                                                                                                    \\ \cmidrule{4-9} 
\multirow{-2}{*}{}                                                                                                         & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Dependence}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Transformation \\ operator\end{tabular}}}} & \multicolumn{1}{c|}{DeepSeek}                     & \multicolumn{1}{c|}{Codellama}                    & \multicolumn{1}{c|}{MagicCoder} & \multicolumn{1}{c|}{DeepSeek}                     & \multicolumn{1}{c|}{Codellama}                    & \multicolumn{1}{c}{MagicCoder} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & Control                                                    & \begin{tabular}[c]{@{}l@{}}Convert \\ For/While\end{tabular}                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.78} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.75} & 0.80                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.57}     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.69}     &    0.63                             \\ \cmidrule{2-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   &                                                            & \begin{tabular}[c]{@{}l@{}}Flip \\ IfElse\end{tabular}                                                             & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.68} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.70} & 0.68                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.52} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.70} & 0.67                            \\ \cmidrule{2-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & Data                                                       & \begin{tabular}[c]{@{}l@{}}Rename \\ variable\end{tabular}                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.62} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.54} & 0.60                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.51} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.62} & 0.49                            \\ \cmidrule{2-9} 
\rowcolor[HTML]{EFEFEF} 
\multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Semantic \\ Preserving \\ Transformation\end{tabular}} &                                                            & \begin{tabular}[c]{@{}l@{}}Reorder \\ parameters\end{tabular}                                                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.65} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.66} & 0.69                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.45} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.62} & 0.50                            \\ \midrule
                                                                                                                           & Control                                                    & \begin{tabular}[c]{@{}l@{}}Replace \\ relational \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.62}                         & \multicolumn{1}{r|}{0.65}                         & 0.59                            & \multicolumn{1}{r|}{0.50}                         & \multicolumn{1}{r|}{0.67}                         & 0.54                            \\ \cmidrule{2-9} 
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Remove \\ conditional \\ statement\end{tabular}                                         & \multicolumn{1}{r|}{0.48}                         & \multicolumn{1}{r|}{0.57}                         & 0.43                            & \multicolumn{1}{r|}{0.38}                         & \multicolumn{1}{r|}{0.52}                         & 0.39                            \\ \cmidrule{2-9} 
                                                                                                                           & Data                                                       & \begin{tabular}[c]{@{}l@{}}Replace \\ arithmetic \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.49}                         & \multicolumn{1}{r|}{0.56}                         & 0.51                            & \multicolumn{1}{r|}{0.38}                         & \multicolumn{1}{r|}{0.63}                         & 0.41                            \\ \cmidrule{2-9} 
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}Semantic \\ Non-Preserving \\ Transformation\end{tabular}}                     &                                                            & \begin{tabular}[c]{@{}l@{}}Remove \\ def \\ statement\end{tabular}                                                 & \multicolumn{1}{r|}{0.50}                         & \multicolumn{1}{r|}{0.64}                         & 0.59                            & \multicolumn{1}{r|}{0.46}                         & \multicolumn{1}{r|}{0.69}                         & 0.45                            \\ \bottomrule
\end{tabular}
}
\end{table}




==> 5.results/tables-backup/rq2_summarization_sematicsimilarity.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{RQ2. The semantic similarity in the summarization of LLMs for the original program and the transformed program}
\label{tab:dependence_concepts}
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{l|l|l|rrr|rrr}
\toprule
                                                                                                                           & \multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{3}{c|}{\textbf{Java}}                                                                                                               & \multicolumn{3}{c}{\textbf{Python}}                                                                                                             \\ \cmidrule{4-9} 
\multirow{-2}{*}{}                                                                                                         & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Dependence}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Transformation \\ operator\end{tabular}}}} & \multicolumn{1}{c|}{\textbf{DeepSeek}}            & \multicolumn{1}{c|}{\textbf{Codellama}}           & \multicolumn{1}{c|}{\textbf{MagicCoder}} & \multicolumn{1}{c|}{\textbf{DeepSeek}}            & \multicolumn{1}{c|}{\textbf{Codellama}}           & \multicolumn{1}{c}{\textbf{MagicCoder}} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Convert \\ For/While\end{tabular}                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.95} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.93} & 0.94                                     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.92}     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.90}     &               0.93                           \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Control}          & \begin{tabular}[c]{@{}l@{}}Flip \\ IfElse\end{tabular}                                                             & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.94} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.66} & 0.93                                     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.95} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.94} & 0.95                                     \\ \cmidrule{2-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Rename \\ variable\end{tabular}                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.88} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.82} & 0.87                                     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.85} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.84} & 0.85                                     \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Semantic \\ Preserving \\ Transformation\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Data}             & \begin{tabular}[c]{@{}l@{}}Reorder \\ parameters\end{tabular}                                                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.93} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.63} & 0.94                                     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.95} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.94} & 0.93                                     \\ \midrule
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ relational \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.94}                         & \multicolumn{1}{r|}{0.93}                         & 0.94                                     & \multicolumn{1}{r|}{0.95}                         & \multicolumn{1}{r|}{0.95}                         & 0.95                                     \\ \cmidrule{3-9} 
                                                                                                                           & \multirow{-2}{*}{Control}                                  & \begin{tabular}[c]{@{}l@{}}Remove \\ conditional \\ statement\end{tabular}                                         & \multicolumn{1}{r|}{0.88}                         & \multicolumn{1}{r|}{0.89}                         & 0.89                                     & \multicolumn{1}{r|}{0.89}                         & \multicolumn{1}{r|}{0.89}                         & 0.89                                     \\ \cmidrule{2-9} 
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ arithmetic \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.92}                         & \multicolumn{1}{r|}{0.60}                         & 0.91                                     & \multicolumn{1}{r|}{0.91}                         & \multicolumn{1}{r|}{0.93}                         & 0.92                                     \\ \cmidrule{3-9} 
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}Semantic \\ Non-Preserving \\ Transformation\end{tabular}}                     & \multirow{-2}{*}{Data}                                     & \begin{tabular}[c]{@{}l@{}}Remove \\ def\\ statement\end{tabular}                                                  & \multicolumn{1}{r|}{0.91}                         & \multicolumn{1}{r|}{0.90}                         & 0.89                                     & \multicolumn{1}{r|}{0.91}                         & \multicolumn{1}{r|}{0.92}                         & 0.90                                     \\ \bottomrule
\end{tabular}
}
\end{table}

==> 5.results/tables-backup/rq2_summarization_tfidf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{RQ2. The similarity in terms of generated tokens in the summarization of LLMs for the original program and the transformed program (TF-IDF)}
\label{tab:dependence_concepts}
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{l|l|l|rrr|rrr}
\toprule
                                                                                                                          &                                                   &                                                                                             & \multicolumn{3}{c|}{\textbf{Java}}                                                                                                      & \multicolumn{3}{c}{\textbf{Python}}                                                                                                    \\ \cmidrule{4-9} 
\multirow{-2}{*}{}                                                                                                        & \multirow{-2}{*}{\textbf{Dependence}}             & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Tranformation\\ operator\end{tabular}}} & \multicolumn{1}{c|}{DeepSeek}                     & \multicolumn{1}{c|}{Codellama}                    & \multicolumn{1}{c|}{MagicCoder} & \multicolumn{1}{c|}{DeepSeek}                     & \multicolumn{1}{c|}{Codellama}                    & \multicolumn{1}{c}{MagicCoder} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                  & \cellcolor[HTML]{EFEFEF}                          & \begin{tabular}[c]{@{}l@{}}Convert \\ For/While\end{tabular}                                & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.89} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.87} & 0.87                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.97}     & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.84}     & 0.84                                \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                  & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Control} & \begin{tabular}[c]{@{}l@{}}Flip \\ IfElse\end{tabular}                                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.86} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.71} & 0.87                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.90} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.90} & 0.90                            \\ \cmidrule{2-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                  & \cellcolor[HTML]{EFEFEF}                          & \begin{tabular}[c]{@{}l@{}}Rename\\ variable\end{tabular}                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.80} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.78} & 0.79                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.78} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.77} & 0.76                            \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Semantic \\ Preserving\\ Transformation\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Data}    & \begin{tabular}[c]{@{}l@{}}Reorder \\ parameters\end{tabular}                               & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.85} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.70} & 0.86                            & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.88} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.87} & 0.87                            \\ \midrule
                                                                                                                          &                                                   & \begin{tabular}[c]{@{}l@{}}Replace \\ relational \\ operator\end{tabular}                   & \multicolumn{1}{r|}{0.87}                         & \multicolumn{1}{r|}{0.89}                         & 0.87                            & \multicolumn{1}{r|}{0.89}                         & \multicolumn{1}{r|}{0.89}                         & 0.89                            \\ \cline{3-9} 
                                                                                                                          & \multirow{-2}{*}{Control}                         & \begin{tabular}[c]{@{}l@{}}Remove \\ conditional \\ statement\end{tabular}                  & \multicolumn{1}{r|}{0.80}                         & \multicolumn{1}{r|}{0.83}                         & 0.80                            & \multicolumn{1}{r|}{0.80}                         & \multicolumn{1}{r|}{0.79}                         & 0.79                            \\ \cline{2-9} 
                                                                                                                          &                                                   & \begin{tabular}[c]{@{}l@{}}Replace \\ arithmetic \\ operator\end{tabular}                   & \multicolumn{1}{r|}{0.85}                         & \multicolumn{1}{r|}{0.67}                         & 0.83                            & \multicolumn{1}{r|}{0.85}                         & \multicolumn{1}{r|}{0.86}                         & 0.85                            \\ \cmidrule{3-9} 
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}Semantic \\ Non-Preserving \\ Transformation\end{tabular}}                    & \multirow{-2}{*}{Data}                            & \begin{tabular}[c]{@{}l@{}}Remove \\ def \\ statement\end{tabular}                          & \multicolumn{1}{r|}{0.83}                         & \multicolumn{1}{r|}{0.84}                         & 0.8                             & \multicolumn{1}{r|}{0.83}                         & \multicolumn{1}{r|}{0.84}                         & 0.81                            \\ \bottomrule
\end{tabular}
}
\end{table}

==> 5.results/tables-backup/rq3.model_size.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{RQ3. The impacts of model sizes on their capability of capturing program semantics}
\label{tab:dependence_concepts}
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{l|l|l|rrr|rrr}
\toprule
                                                                                                                           & \multicolumn{1}{c|}{}                                      & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{3}{c|}{\textbf{Exactly match}}                                                                                               & \multicolumn{3}{c}{\textbf{F1-Score}}                                                                                                    \\ \cmidrule{4-9} 
\multirow{-2}{*}{}                                                                                                         & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Dependence}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Transformation \\ operator\end{tabular}}}} & \multicolumn{1}{c|}{DeepSeek-1.3B}                & \multicolumn{1}{c|}{DeepSeek-6.7B}                & \multicolumn{1}{c|}{DeepSeek-33B} & \multicolumn{1}{c|}{DeepSeek-1.3B}                & \multicolumn{1}{c|}{DeepSeek-6.7B}                & \multicolumn{1}{c}{DeepSeek-33B} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Convert \\ For/While\end{tabular}                                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.68} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.72} & 0.81                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.87} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.85} & 0.87                              \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Control}          & \begin{tabular}[c]{@{}l@{}}Flip \\ IfElse\end{tabular}                                                             & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.53} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.80} & 0.50                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.78} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.91} & 0.69                              \\ \cmidrule{2-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Rename \\ variable\end{tabular}                                                         & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.25} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.34} & 0.43                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.54} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.62} & 0.67                              \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Semantic \\ Preserving \\ Transformation\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Data}             & \begin{tabular}[c]{@{}l@{}}Reorder \\ parameters\end{tabular}                                                      & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.69} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.72} & 0.65                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.85} & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.88} & 0.79                              \\ \midrule
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ relational \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.51}                         & \multicolumn{1}{r|}{0.45}                         & 0.44                              & \multicolumn{1}{r|}{0.76}                         & \multicolumn{1}{r|}{0.70}                         & 0.67                              \\ \cmidrule{3-9} 
                                                                                                                           & \multirow{-2}{*}{Control}                                  & \begin{tabular}[c]{@{}l@{}}Remove \\ conditional \\ statement\end{tabular}                                         & \multicolumn{1}{r|}{0.32}                         & \multicolumn{1}{r|}{0.39}                         & 0.37                              & \multicolumn{1}{r|}{0.61}                         & \multicolumn{1}{r|}{0.58}                         & 0.56                              \\ \cline{2-9} 
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ arithmetic \\ operator\end{tabular}                                          & \multicolumn{1}{r|}{0.46}                         & \multicolumn{1}{r|}{0.49}                         & 0.40                              & \multicolumn{1}{r|}{0.71}                         & \multicolumn{1}{r|}{0.66}                         & 0.58                              \\ \cmidrule{3-9} 
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}Semantic \\ Non-Preserving \\ Transformation\end{tabular}}                     & \multirow{-2}{*}{Data}                                     & \begin{tabular}[c]{@{}l@{}}Remove \\ def \\ statement\end{tabular}                                                 & \multicolumn{1}{r|}{0.51}                         & \multicolumn{1}{r|}{0.51}                         & 0.60                              & \multicolumn{1}{r|}{0.75}                         & \multicolumn{1}{r|}{0.75}                         & 0.76                              \\ \bottomrule
\end{tabular}
}
\end{table}

==> 5.results/tables-backup/rq4_correlation_correctness.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\caption{RQ4. The correlation between the code understanding of LLMs and the correctness of its generated code}
\label{tab:dependence_concepts}
\resizebox{1.5\columnwidth}{!}{%
\begin{tabular}{l|l|l|rr|rr|rr}
\toprule
                                                                                                                           & \multicolumn{1}{c|}{}                                      &                                                                                              & \multicolumn{2}{c|}{\textbf{DeepSeek}}                                                                                                                              & \multicolumn{2}{c|}{\textbf{Codellama}}                                                                                                                             & \multicolumn{2}{c}{\textbf{MagicCoder}}                                                                                                                            \\ \cmidrule{4-9} 
\multirow{-2}{*}{}                                                                                                         & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Dependence}}} & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Transformation\\ operator\end{tabular}}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Correct \\ program\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Incorrect \\ program\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Correct \\ program\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Incorrect \\ program\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Correct \\ program\end{tabular}} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Incorrect \\ program\end{tabular}} \\ \midrule
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Convert \\ For/While\end{tabular}                                 & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.72}                               & 0.82                                                                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.76}                               & 0.82                                                                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.86}                               & 0.84                                                                              \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Control}          & \begin{tabular}[c]{@{}l@{}}Flip \\ IfElse\end{tabular}                                       & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.84}                               & 0.58                                                                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.63}                               & 0.58                                                                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.75}                               & 0.90                                                                              \\ \cmidrule{2-9} 
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF}                                                                                                   & \cellcolor[HTML]{EFEFEF}                                   & \begin{tabular}[c]{@{}l@{}}Rename \\ variable\end{tabular}                                   & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.37}                               & 0.35                                                                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.51}                               & 0.35                                                                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.56}                               & 0.46                                                                              \\ \cmidrule{3-9} 
\rowcolor[HTML]{EFEFEF} 
\multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}l@{}}Semantic \\ Preserving \\ Transformation\end{tabular}} & \multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}Data}             & \begin{tabular}[c]{@{}l@{}}Reorder \\ parameters\end{tabular}                                & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.73}                               & 0.52                                                                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.67}                               & 0.52                                                                              & \multicolumn{1}{r|}{\cellcolor[HTML]{EFEFEF}0.65}                               & 0.61                                                                              \\ \midrule
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ relational \\ operator\end{tabular}                    & \multicolumn{1}{r|}{0.48}                                                       & 0.53                                                                              & \multicolumn{1}{r|}{0.53}                                                       & 0.53                                                                              & \multicolumn{1}{r|}{0.67}                                                       & 0.49                                                                              \\ \cmidrule{3-9} 
                                                                                                                           & \multirow{-2}{*}{Control}                                  & \begin{tabular}[c]{@{}l@{}}Remove \\ conditional \\ statement\end{tabular}                   & \multicolumn{1}{r|}{0.41}                                                       & 0.33                                                                              & \multicolumn{1}{r|}{0.40}                                                       & 0.33                                                                              & \multicolumn{1}{r|}{0.44}                                                       & 0.30                                                                              \\ \cmidrule{2-9} 
                                                                                                                           &                                                            & \begin{tabular}[c]{@{}l@{}}Replace \\ arithmetic \\ operator\end{tabular}                    & \multicolumn{1}{r|}{0.49}                                                       & 0.40                                                                              & \multicolumn{1}{r|}{0.52}                                                       & 0.40                                                                              & \multicolumn{1}{r|}{0.44}                                                       & 0.44                                                                              \\ \cmidrule{3-9} 
\multirow{-4}{*}{\begin{tabular}[c]{@{}l@{}}Semantic \\ Non-Preserving \\ Transformation\end{tabular}}                     & \multirow{-2}{*}{Data}                                     & \begin{tabular}[c]{@{}l@{}}Remove \\ def \\ statement\end{tabular}                           & \multicolumn{1}{r|}{0.56}                                                       & 0.66                                                                              & \multicolumn{1}{r|}{0.73}                                                       & 0.66                                                                              & \multicolumn{1}{r|}{0.6}                                                        & 0.42                                                                              \\ \bottomrule
\end{tabular}
}
\end{table}

==> 5.results/tables/rq3.model_size.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{RQ3. The impacts of model sizes on their capability of capturing code semantics}
\label{tab:model_size}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|l|r|r|rr}\toprule
\multicolumn{2}{c|}{} &\textbf{Deepseek1.3} &\textbf{DeepSeek6.7} &\textbf{DeepSeek33} \\\midrule
\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Code \\ summarization\end{tabular}} &Robustness &0.92 &0.93 &0.93 \\ 
&Sensitivity &0.09 &0.09 &0.09 \\\midrule
\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Method name \\ prediction\end{tabular}} &Robustness &0.54 &0.65 &0.60 \\
&Sensitivity &0.55 &0.54 &0.55 \\\midrule
\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Output \\ prediction\end{tabular}} &Robustness &0.64 &0.69 &0.68 \\
&Sensitivity &0.46 &0.48 &0.49 \\
\bottomrule
\end{tabular}
}
\end{table}

==> 5.results/tables/rq4_correlation_correctness.tex <==


%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{RQ4. The correlation between the code understanding of Code LLMs and the correctness of its generated code}
\label{tab:correstness_correlation}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|rr|rr|rrr}\toprule
\textbf{} &\multicolumn{2}{c|}{\textbf{DeepSeek}} &\multicolumn{2}{c|}{\textbf{Codellama}} &\multicolumn{2}{c}{\textbf{MagicCoder}} \\\midrule
&\begin{tabular}[c]{@{}c@{}}Correct \\ program\end{tabular} &\begin{tabular}[c]{@{}c@{}}Incorrect \\ program\end{tabular} &\begin{tabular}[c]{@{}c@{}}Correct \\ program\end{tabular} &\begin{tabular}[c]{@{}c@{}}Incorrect \\ program\end{tabular}  &\begin{tabular}[c]{@{}c@{}}Correct \\ program\end{tabular} &\begin{tabular}[c]{@{}c@{}}Incorrect \\ program\end{tabular} \\ \midrule
\textbf{Robustness} &0.67 &0.57 &0.64 &0.57 &0.71 &0.70 \\
\textbf{Sensitivity} &0.52 &0.52 &0.46 &0.52 &0.46 &0.59 \\
\bottomrule
\end{tabular}
}
\end{table}

==> 7.related_work.tex <==
\section{Related Work}

\subsection{Code LLMs}

With the development LLMs, multiple models have been specialized for code which demonstrates substantial capabilities in a variety of SE tasks.  

\subsection{Evaluating Code LLMs}
